Optimal Threshold Design for Quanta Image Sensor

Quanta Image Sensor (QIS) is a binary imaging device envisioned to be the next generation image sensor after CCD and CMOS. Equipped with a massive number of single photon detectors, the sensor has a threshold $q$ above which the number of arriving photons will trigger a binary response "1", or "0" otherwise. Existing methods in the device literature typically assume that $q=1$ uniformly. We argue that a spatially varying threshold can significantly improve the signal-to-noise ratio of the reconstructed image. In this paper, we present an optimal threshold design framework. We make two contributions. First, we derive a set of oracle results to theoretically inform the maximally achievable performance. We show that the oracle threshold should match exactly with the underlying pixel intensity. Second, we show that around the oracle threshold there exists a set of thresholds that give asymptotically unbiased reconstructions. The asymptotic unbiasedness has a phase transition behavior which allows us to develop a practical threshold update scheme using a bisection method. Experimentally, the new threshold design method achieves better rate of convergence than existing methods.

==> customFigureMacros.tex <==
% ===========================================================
% Definitions, commands and environnments for drawing figures
%
% Vivek Goyal
% based on work by
% Ivana Jovanovic, Patrick Vandewalle, Olivier Roy - 2005
% ===========================================================

% --------
% PACKAGES
% --------
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{ifthen}
%\RequirePackage{pstricks}
%\RequirePackage{pst-plot}
%\RequirePackage{algo}
%\RequirePackage{epsfig}
%\RequirePackage{latexsym}
%\RequirePackage{subfigure}

% --------------------
% PSTRICKS DEFINITIONS
% --------------------
% Upsampling operation (reference point at the center of the circle)
% Parameter #1: upsampling factor
\def\upsampling#1{

    \pscircle(0,0){0.5}
    \psline{->}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Downsampling operation (reference point at the center of the circle)
% Parameter #1: downsampling factor
\def\downsampling#1{

    \pscircle(0,0){0.5}
    \psline{<-}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Sampling operation (reference point at the center of the box)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\sampler#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.6,-0.2)(-0.2,-0.2)
    \psline{-}(0.2,-0.2)(0.6,-0.2)
    \psline{-}(-0.2,-0.2)(0.1,0.1)
    \rput(-0.3,0.3){#1}

}

% Discrete-to-continuous operation (reference point at the center of the box)
% (Generation of weighted Dirac train)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\diracTrain#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.8,0)(0.8,0)
    \psline{->}(-0.6,0)(-0.6,-0.45)
    \psline{->}(-0.3,0)(-0.3,-0.3)
    \psline{->}( 0.0,0)( 0.0, 0.4)
    \psline{->}( 0.3,0)( 0.3, 0.4)
    \psline{->}( 0.6,0)( 0.6,-0.35)
    \rput(0.3,-0.2){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\filter#1{

    \psframe(-1,-0.5)(1,0.5)
    \rput(0,0){#1}

}

\def\shortfilter#1{

    \psframe(-0.75,-0.5)(0.75,0.5)
    \rput(0,0){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\widefilter#1{

    \psframe(-2,-0.5)(2,0.5)
    \rput(0,0){#1}

}

% Sum (reference point at the center of the circle)
\def\sumsymbol{

    \pscircle(0,0){0.25}
    \rput(0,0){$+$}

}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\analysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\downsampling{#2}}
    \psline{-}(4,0)(4.5,0)
}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\wideanalysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(2.5,0){\widefilter{#1}}
    \psline{-}(4.5,0)(5,0)
    \rput(5.5,0){\downsampling{#2}}
    \psline{-}(6,0)(6.5,0)
}

% Synthesis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: synthesis filter label
% Parameter #2: upsampling factor
\def\synthesis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(3,0){\filter{#1}}
    \psline{-}(4,0)(4.5,0)
}

% Filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: synthesis filter label
% Parameter #3: down/upsampling factor
\def\filterbankchannel#1#2#3{

    \rput(0,0){\analysis{#1}{#3}}
    \rput(4.5,0){\synthesis{#2}{#3}}

}

% Two channel filter bank (reference point at the begining of the filter bank)
% Parameter #1: lowpass analysis filter label
% Parameter #2: lowpass synthesis filter label
% Parameter #3: highpass analysis filter label
% Parameter #4: highpass synthesis filter label

\def\twochannelfilterbank#1#2#3#4{

    % Input
    \psline{*-}(0,0)(0.5,0)
    \psline{-}(0.5,-0.75)(0.5,0.75)

    % Highpass branch
    \rput(0.5,0.75){\filterbankbranch{#3}{#4}{2}}

    % Lowpass branch
    \rput(0.5,-0.75){\filterbankbranch{#1}{#2}{2}}

    % Output
    \psline{->}(9.5,0.75)(9.5,0.25)
    \rput(9.5,0){\sumsymbol}
    \psline{->}(9.5,-0.75)(9.5,-0.25)
    \psline{-*}(9.75,0)(10.25,0)

}




% Parameter #1: filter label
% Parameter #2: sampling factor
% Parameter #3: delay
\def\mybranch#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(2.75,0){\shortfilter{#3}}
    \psline{-}(3.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchA#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}


\def\mybranchB#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(4.5,0)
    \rput(5.25,0){\shortfilter{#3}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchC#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}
